Exponential Integrators with Parallel-in-Time Rational Approximations for the Shallow-Water Equations on the Rotating Sphere

High-performance computing trends towards many-core systems are expected to continue over the next decade. As a result, parallel-in-time methods, mathematical formulations which exploit additional degrees of parallelism in the time dimension, have gained increasing interest in recent years. In this work we study a massively parallel rational approximation of exponential integrators (REXI). This method replaces a time integration of stiff linear oscillatory and diffusive systems by the sum of the solutions of many decoupled systems, which can be solved in parallel. Previous numerical studies showed that this reformulation allows taking arbitrarily long time steps for the linear oscillatory parts. The present work studies the non-linear shallow-water equations on the rotating sphere, a simplified system of equations used to study properties of space and time discretization methods in the context of atmospheric simulations. After introducing time integrators, we first compare the time step sizes to the errors in the simulation, discussing pros and cons of different formulations of REXI. Here, REXI already shows superior properties compared to explicit and implicit time stepping methods. Additionally, we present wallclock-time-to-error results revealing the sweet spots of REXI obtaining either an over 6x higher accuracy within the same time frame or an about 3x reduced time-to-solution for a similar error threshold. Our results motivate further explorations of REXI for operational weather/climate systems.

==> 10_03_error_vs_linear_oscillatory_stiffness.tex <==

\subsection{Linear vs. nonlinear oscillatory stiffness}

\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{benchmarks_sphere/parco_jrn_parco_rexi_nonlinear__compare_dt_vs_accuracy_modified_galewsky/output_plotting_runtime-timestep-size_vs_sphere-data-diff-prog-h-res-norm-linf}
	\end{center}
	\caption{
		\label{fig:compare_dt_vs_accuracy_modified_galewsky}
		REXI time integration method for barotropic instability benchmark comparing the accuracy dependency on the time step size and linear oscillatory stiffness.
		For stronger stiffness (larger $h_0$), we see also an increase in errors.
	}
\end{figure}


All previous studies were conducted with a similar ratio of stiffness\footnote{We consider stiffness in terms of its oscillatory behaviour, see also \cite{CoxMathews2002}.} between the linear and non-linear terms.
In this section, we vary this ratio in order to investigate the sensitivity of REXI.
We accomplish this by scaling the average geopotential $\overline{\Phi} = g \overline h$ via the surface height which linearly relates to it.
For the linear operator $L_g$, this geopotential is linearly related to its stiffness.
Therefore, we vary this geopotential from $\overline{\Phi} \in \{ 2, 4, \ldots, 18\} \cdot 10^3 g$ with $\Phi=10^4 g$ the parameter used in the barotropic instability benchmark.
The results for this are given in Fig.\,\ref{fig:compare_dt_vs_accuracy_modified_galewsky}.




Despite REXI being able to time-integrate the linear parts with very high accuracy, the time integration over 5 days in total as well as the interactions with the non-linear parts introduce more errors with increasing frequency of the linear operator and vice versa.
We can observe the 

==> test <==
\nth{2}
\nth{2}
3rd


==> test.tex <==
\subsection{Nomenclature for time splitting methods}


\begin{table*}
	\center
	\begin{center}
		\begin{tabular}{|c|l|l|}
		\hline
			\textbf{Symbol}		&	\textbf{Description}	&	\textbf{ID}\\
		\hline
		\hline
			$L_g$	&	Linear wave motions induced by gravitational force	&	\texttt{lg}	\\
		\hline
			$L_c$	&	Coriolis effect acting on velocity components	&	\texttt{lc}	\\
		\hline
			$L = L_g + L_c$	&	Both linear terms&	\texttt{l}	\\
		\hline
			$N$		&	Non-linear advection and divergence				&	\texttt{n}\\
		\hline
		\end{tabular}
		\caption{\label{tbl:swe_terms}
			Description and string identifiers of different terms in the shallow-water equations on the rotating sphere.}
	\end{center}
\end{table*}


\begin{table*}
\center
\begin{tabular}{|l|c|}
	\hline
	Time stepping 			&Identifier\\
	\hline
	\hline
	\nth{2} order explicit Runge-Kutta		&\texttt{erk}\\
	\hline
	Crank-Nicolson			&\texttt{irk}\\
	\hline
	REXI						&\texttt{rexi}\\
	\hline
	Exponential Time Differencing Runge-Kutta	&\texttt{etdrk}\\
	\hline
\end{tabular}
\caption{\label{tbl:time_integrators_names}
	Description and string identifiers of different time integrators used throughout this work.
}
\end{table*}

We briefly introduce a string annotation to differentiate between the implementations of the time splitting methods.
Section \ref{sec:shallow_water_equations} introduced the different terms $L_g$, $L_c$, $N$ of the SWE PDE.
These terms will be denoted as \texttt{lg}, \texttt{lc}, \texttt{n}, respectively, and an overview is given in Table \ref{tbl:swe_terms}.
Abbreviations for different single-step time integrators used in this work are given in Table \ref{tbl:time_integrators_names}.
We use a concatenation of operators followed by the time stepping method to denote them.
E.g.\,using a Strang-splitting where the linear term is assumed to be $L_g$ and treated by a Crank-Nicolson scheme and the other non-linear terms assumed to be the Coriolis $L_c$ and non-linear terms $N$ and treated by an explicit \nth{2} order Runge-Kutta is denoted by \texttt{lg\_irk\_lc\_n\_erk\_ver0} where \texttt{ver0} denotes the version integrating the linear parts twice in each time step, see Sec.\,\ref{sec:strang_splitting}.

test 
\new{\textbf{test}}
\new{a\textbf{test}}
a\textbf{test}b
a\textbf{test}bb\textbf{test}bb
a\textbf{test}b
b\textbf{test}bb



For ETD2RK, non-linearities are natively supported and no Strang-splitting is needed to gain a \nth{2} order accurate method.
This is denoted e.g.\,as \texttt{lg\_rexi\_lc\_n\_etdrk} which would treat the term $L_g$ as the only linear one with REXI and the terms $L_c + N$ as the non-linear ones within the ETD2RK time integration (see Sec.\,\ref{sec:etdnrk}).


followup text with \textbf{bold} face text
